Optimizing Microservices Placement in the Cloud-to-Edge Continuum: A Comparative Analysis of App and Service Based Approaches

In the ever-evolving landscape of computing, the advent of edge and fog computing has revolutionized data processing by bringing it closer to end-users. While cloud computing offers numerous advantages, including mobility, flexibility and scalability, it introduces challenges such as latency. Fog and edge computing emerge as complementary solutions, bridging the gap and enhancing services' proximity to users. The pivotal challenge addressed in this paper revolves around optimizing the placement of application microservices to minimize latency in the cloud-to-edge continuum, where a proper node selection may influence the app's performance. Therefore, this task gains complexity due to the paradigm shift from monolithic to microservices-based architectures. Two distinct placement approaches, app-based and service-based, are compared through four different placement algorithms based on criteria such as link latency, node resources, and gateway proximity. App-based allocates all the services of one app sequentially, while service-based allocates one service of each app at a time. The study, conducted using YAFS (Yet Another Fog Simulator), evaluates the impact of these approaches on latency and load balance. The findings consistently confirm the hypothesis that strategies utilizing a service-based approach outperformed or performed equally well compared to app-based approaches, offering valuable insights into trade-offs and performance differences among the algorithms and each approach in the context of efficient microservices placement in cloud-to-edge environments.

==> pseudo_code/RR_IPT_placement_v3.tex <==
%not in use!!!
\begin{algorithm}[H]
	\caption{RR\_IPT} 
	\begin{algorithmic}[1]
            \State generate louvain communities
            \State sort communities by IPT sum
            \State sort community nodes by IPT
            \State sort apps by messages sum
            \State $appsPerComm \gets $ len(self.appJson) // comms\_nr
            \State $appsCount \gets $ [0] * comms\_nr

            \For {$app\_i=0,\ldots, appsNum$}
                \State $commSearch \gets $0
                \State $node\_i \gets $0
                \While {$node\_i < len(apps)$}
                    \State allocate service on the first node possible of the first community
                    \If{$didAlloc$}
                        \State append it and those before to the end of the array
                    \Else
                        \State clear all current app allocation

                        \If{$commSearch \geq commsNum$}
                            \State allocate app in cloud
                            \State break
                        \Else
                            \State append current community to the end of the array
                            \State $node\_i \gets $0
                            \State $commSearch \gets $commSearch+1
                        \EndIf
                      
                    % \Else
                    \EndIf
                \EndWhile
                \State appsCount[0] += 1
                \If {$appsCount[0] \geq appsPerComm$}
                    \State append current community to the end of the array
                \EndIf
                
            \EndFor
  
  
  
  
  
  
            % \For {$iteration=1,2,\ldots$}
		% 	\For {$actor=1,2,\ldots,N$}
			%	\State Run policy $\pi_{\theta_{old}}$ in environment for $T$ time steps
				%\State Compute advantage estimates $\hat{A}_{1},\ldots,\hat{A}_{T}$
			%\EndFor
			%\State Optimize surrogate $L$ wrt. $\theta$, with $K$ epochs and minibatch size $M\leq NT$
			%\State $\theta_{old}\leftarrow\theta$
		%\EndFor
	\end{algorithmic} 
\end{algorithm}

